Expectations, Explanations, and Embodiment: Attempts at Robot Failure Recovery

Expectations critically shape how people form judgments about robots, influencing whether they view failures as minor technical glitches or deal-breaking flaws. This work explores how high and low expectations, induced through brief video priming, affect user perceptions of robot failures and the utility of explanations in HRI. We conducted two online studies ($N=600$ total participants); each replicated two robots with different embodiments, Furhat and Pepper. In our first study, grounded in expectation theory, participants were divided into two groups, one primed with positive and the other with negative expectations regarding the robot's performance, establishing distinct expectation frameworks. This validation study aimed to verify whether the videos could reliably establish low and high-expectation profiles. In the second study, participants were primed using the validated videos and then viewed a new scenario in which the robot failed at a task. Half viewed a version where the robot explained its failure, while the other half received no explanation. We found that explanations significantly improved user perceptions of Furhat, especially when participants were primed to have lower expectations. Explanations boosted satisfaction and enhanced the robot's perceived expressiveness, indicating that effectively communicating the cause of errors can help repair user trust. By contrast, Pepper's explanations produced minimal impact on user attitudes, suggesting that a robot's embodiment and style of interaction could determine whether explanations can successfully offset negative impressions. Together, these findings underscore the need to consider users' expectations when tailoring explanation strategies in HRI. When expectations are initially low, a cogent explanation can make the difference between dismissing a failure and appreciating the robot's transparency and effort to communicate.

==> sections/01_Introduction_old.tex <==
\section{Introduction}
% \elmira{@ALL Please look at the new plots and color codes and put your comments}



% \irmak{
% Here, I tried to emphasize the novelty of evaluating the impacts of explanations based on user expectations. Hope it conveys well, feel free to change as you wish :) Also, I would like to discuss the last two sentences about results. For me, this was the most important takeaway of the paper, but I am unsure if you would agree
% %Points to make: 

% %explanations are critical

% %they should be based on user expectations

% %what is missing? Do not account for user expectations
% %What do we do: Prime people, generate explanations, observe the impact of such explanations
% }

%new one
When robots operate in human environments, user expectations play a crucial role in shaping human-robot interaction (HRI)~\citep{dogan2024grace} and can significantly influence how people interpret and accept robot explanations. For instance, one user might be very familiar with robots and view them as helpful assistants, expecting the robot to act proactively and autonomously. On the other hand, another user might have concerns about potential errors made by robots and prefer the robot to act more cautiously, providing detailed explanations and seeking user approval before taking any action. This variation in user preconception can significantly influence how users perceive and react to the robot's explanations, making it essential to explore whether and how these differences affect human-robot interaction.

%old one
%When robots operate in human environments, providing explanations for robot decisions improves users trust towards robots~\citep{siau2018building, edmonds2019tale, barredoarrieta2020ExplainableArtificialIntelligence, doi:10.1177/15553434221136358} as well as the effectiveness of human-robot interaction (HRI)~\citep{sridharan2019towards, setchi2020explainable}. User expectations, meanwhile, play a crucial role in shaping these interactions and can significantly influence how people interpret and accept robot explanations.
%For instance, one user might be very familiar with robots and view them as helpful assistants, expecting the robot to act proactively and autonomously. On the other hand, another user might have concerns about potential errors made by robots and prefer the robot to act more cautiously, providing detailed explanations and seeking user approval before taking any action.
%This variation in user priming can significantly influence how users perceive and react to the robot's explanations, making it essential to tailor robots' communication strategies based on user expectations.
%This variation in user conditioning %priming
%can significantly influence how users perceive and react to the robot's explanations, making it essential to explore whether and how these differences affect human-robot interaction.
%This variation in user priming can significantly influence how users perceive and accept the robot's explanations, making it essential to investigate robots' communication strategies based on user expectations and priming.
%Former literature has explored the impacts of providing robot explanations in varying forms~\citep{edmonds2019tale}, such as providing visual explanations for robot decisions~\citep{}, communicating through verbal explanations~\citep{han2021need} and leveraging explanations in follow-up questions~\citep{9889368, dougan2023leveraging}. Although these studies have shown pioneering results demonstrating the impacts of providing explanations, they have not accounted for individuals' expectations and their priming about robot capabilities while generating robot explanations. \textit{To bridge this gap, our study is the first to explore how people's priming about robots affects their perception of robot explanations.}
% \begin{figure}[t]
%     \centering
%     \begin{minipage}{0.24\textwidth}
%         \centering
%         \includegraphics[height=0.09\textheight]{figures/peppervid.png}
%         %\caption*{Pepper setting.}
%     \end{minipage}
%     \begin{minipage}{0.24\textwidth}
%         \centering
%         \includegraphics[height=0.09\textheight]{figures/furhatvid.png}
%         %\caption*{Furhat setting.}
%     \end{minipage}
%     \caption{Priming scenario with Pepper (left) and Furhat (right)}
%     \label{fig:video_setting}
% \end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/Priming_videos.png}
    \caption{Priming scenario with Pepper (left) and Furhat (right)}
    \label{fig:video_setting}
\end{figure}

% \elmira{@Iramk could you add a paragraph here related to research on expectations in robotics. Example from this paper (a framework for studying users' expectations of social robots was developed by \citep{relatedwork_expectation_evaluation_framework})}
% \irmak{re @Elmira, combined it with the explainability literature, let me know how it sounds. I also changed the first paragraph to focus more on user expectations.}

Previous research has highlighted the common mismatch between user expectations and the actual capabilities of social robots~\citep{relatedwork_expectation_evaluation_framework}, a gap that often leads to disappointment and can diminish the quality of interactions~\citep{relatedwork_expectation_Expectancies,kruglanski2007principles}. A promising approach for addressing this gap can be through providing explanations for robot mistakes, helping to align users' expectations with the robot's actual capabilities. In line with this, previous work has explored various ways of delivering robot explanations~\citep{edmonds2019tale}, including visual explanations for robot decisions~\citep{dougan2023leveraging, sobrin2024enhancing}, conveying explanations through verbal interaction~\citep{han2021need, stange2022self}, and such explanations incorporated into follow-up questions~\citep{9889368} and used for clarifying robot failures~\citep{han2021need, das2021ExplainableAIRobot}. While these studies have provided valuable insights into the impact of robot explanations while handling robot mistakes, they have not considered individuals' expectations and preconceptions regarding robot capabilities during the explanation generation process. \textit{To address this challenge, our study is the first to examine how people's expectations affect their perception of robot explanations.}


%old one
%Previous research has investigated the effects of providing robot explanations in various forms~\citep{edmonds2019tale}, such as visual explanations for robot decisions~\citep{dougan2023leveraging, sobrin2024enhancing}, conveying through verbal interaction~\citep{han2021need, stange2022self}, and such explanations incorporated into follow-up questions~\citep{9889368} and used for clarifying robot failures~\citep{han2021need, das2021ExplainableAIRobot}. While these studies have provided valuable insights into the impact of robot explanations while handling robot mistakes, they have not considered individuals' expectations and their preconception 
%priming 
%regarding robot capabilities during the explanation generation process. \textit{To address this gap, our study is the first to examine how people's expectations affect their perception of robot explanations.}

In this paper, we investigate how priming people about robots' capabilities influences people's perception of robots, 
%interaction, 
particularly in the context of recovering from robot mistakes through the use of explanations. Our approach involves conducting two sets of user studies repeated with two different robots (Pepper and Furhat) to explore how varying robotic features and tasks influence user perceptions of explanations. Initially, participants were primed with either high or low expectations for the robots' capabilities (e.g., the robots performing the task flawlessly versus making errors) to establish varied expectations. Subsequently, to evaluate the effect of these primed expectations on how robot explanations are perceived, the robots deliberately made errors during a second task, and they either provided explanations for their mistakes or omitted any explanations. Our results show that the priming study successfully set high or low expectations about robot capabilities, and critically, when these expectations were low, providing explanations was helpful in enhancing the robot's perceived level of expressiveness, specifically for the Furhat robot. Subsequently, people's perception of the robot was improved when it explained the reasons for its mistakes.
%the priming study successfully shapes people's perception of the capability of the robot and....   

==> sections/02_Related_Work_old.tex <==
\nopagebreak
\section{Related Work}
\subsection{Expectations for Robots}
``Expectation'' is a psychological concept that refers to an individual's anticipation of outcomes based on cognitive processes, which guide behaviour, hopes, and intentions \citep{relatedwork_expectation_Expectancies,kruglanski2007principles}. 
% Neuroscience research has demonstrated that expectations arise from specialized cognitive networks and influence automatic behaviours and comprehension during interactions \citep{relatedwork_expectation_defination,relatedwork_expectation_neuroscience}. 
In social contexts, including HRI, individuals naturally form expectations that simplify the processing of familiar social situations~\citep{relatedwork_expectation_situation_role_in_HRI} while making unexpected behaviours more challenging to interpret \citep{relatedwork_expectation_role_in_HRI}.
%Therefore, it is crucial to understand how users' expectations affect their perception of designing robots that meet these anticipations. 
Users hope robots recognize and align with their expectations in various interaction roles \citep{relatedwork_expectation_situation_role_in_HRI}. 
Several studies have explored these expectations, focusing on robot appearance \citep{relatedwork_expectation_robot_appearance} and interaction abilities \citep{relatedwork_expectation_robot_interaction_skill}.
% , which have shown that participants’ expectations are shaped by the interaction itself rather than by the specific type of social robot involved \citep{relatedwork_expectation_meister2014robot}.

A study by Edwards et al.   \citep{relatedwork_expectation_initialize_HHI} has shown that compared to Human-Human Interactions (HHI), users tend to have more uncertain and lower expectations of robots. These expectations are dynamic and can be changed based on several factors. For example, perceived interaction skills may shift depending on the user’s anticipated future role for the robot \citep{relatedwork_expectation_robot_interaction_skill}. To examine how expectations impact interaction, a framework for studying users' expectations of robots was developed by Rosen et al. \citep{relatedwork_expectation_evaluation_framework}, focusing on affect, cognitive processing, and performance. However, there is still a mismatch between the expected and actual capabilities of robots, leading to potential disappointment and negative effects \citep{relatedwork_expectation_Expectancies,kruglanski2007principles,relatedwork_expectation_evaluation_framework}. Therefore, reducing the gap between expectations and reality is key to fostering long-term relationships, affecting users' evaluation with robots \citep{relatedwork_expectation_jokinen2017expectations}. 
%Some research has also addressed strategies for managing expectations in specific domains, such as child-robot interaction \citep{relatedwork_expectation_chilren_management}. 




% \begin{figure}[htp]
%     \centering
%     \includegraphics[width=0.4\textwidth]{figures/taxonomy.jpg}
%     \caption{A human-robot failure taxonomy. Adapted from \citep{honig2018understanding}. \elmira{We remove this and mention it in the text}}
%     \label{tax}
% \end{figure}

\subsection{Priming and Expectations}
Priming is a non-conscious process associated with learning, where exposure to a priming stimulus influences the response to a subsequent target stimulus \citep{relatedwork_priming_hri}. For instance, ``movement priming'' refers to how one's movement can affect another person's actions or their own future movements \citep{relatedwork_priming_defination}. 

%Previous studies have explored various types of priming, including semantic \citep{relatedwork_priming_senmatic_meyer1971facilitation, relatedwork_priming_senmatic_schvaneveldt1973retrieval, relatedwork_priming_senmatic_schvaneveldt1976lexical}, stereotype \citep{relatedwork_priming_sterotype_abs}, affective \citep{relatedwork_priming_affective_abshermans2003affective, relatedwork_priming_affective_klauer2003affective, relatedwork_priming_affective_murphy1993affect, relatedwork_priming_affective_tamietto2010neural}, visual \citep{relatedwork_priming_visual_gauthier2000visual}, and motor priming \citep{relatedwork_priming_motion_craighero2002hand, relatedwork_priming_motion_craighero1998visuomotor}.

% Studies that use priming in HRI are still limited even though it is considered to have a significant impact on user expectations and behaviour \citep{relatedwork_priming_hri}.
Priming in HRI is considered to have a significant impact on user expectations and behavior \citep{relatedwork_priming_hri}. Initial interactions or information about a robot can shape users' expectations and perceptions of its capabilities, potentially creating an ``expectation gap'' if the robot fails to meet these anticipations, which can affect user's satisfaction \citep{relatedwork_priming_hri}. Therefore, priming offers a possible strategy for designing more effective HRI experiences. 
%Therefore, it is possible to incorporate priming to develop effective HRI strategies. 
For example, Liao and MacDonald \citep{relatedwork_priming_affectivepriming}  explored how emotional priming impacts user perception in autonomous products, showing the potential to build long-term relationships via affective priming.
% Another study investigated how explicit and implicit emotional attributions to robots influence perceptions of their anthropomorphism, revealing that both types of emotional attribution were linked to perceptions of robot warmth and competence, providing insights into how emotional priming affects robot perception in HRI \citep{relatedwork_priming_SPATOLA2021106934}. 
Additionally, research on media representations of robot characters has shown that sympathetic portrayals in media can prime positive social evaluations of robots, influencing individuals' mental models and social assessments \citep{relatedwork_priming_media}. 
% \elmira{There was also a paper which used priming people about AI in the medical field; it is worth mentioning here. ``How are radiologists' decisions impacted by AI
% suggestions? Moderating effect of explainability
% inputs and attitudinal priming in examining
% mammograms''}
Moreover, another study \citep{mehrizi2022radiologists} examined the impact of priming on decision-making processes in medical contexts, revealing that the effects of explainability inputs and attitudinal priming are limited in mitigating the unintended influence of incorrect algorithmic suggestions.



\subsection{Robot Capabilities and Failures}
In recent years, many social robots have been developed for a wide range of HRI scenarios, particularly in customer service, healthcare, and educational settings. Two commonly used robots in these domains are Pepper and Furhat.
Pepper \citep{softbankpepper} is a humanoid robot equipped with cameras, a 3D sensor, and microphones, enabling it to perceive its surroundings and respond verbally or with body gestures. The mobile base allows it to move around, adopt various postures, and handle objects. However, its facial expression remains static, and its mouth does not move when speaking.
Furhat \citep{furhatrobotics} is a conversational robot with a back-projected, human-like face capable of displaying a wide range of facial expressions like nodding, head-shaking, and raising eyebrows. Its design allows for customizing various genders, ages, skin tones, and voices with different speaking styles. However, it lacks mobility and the ability to adopt body postures since it is a head-shaped robot without a mobile body.

Robots not only have capabilities and limitations, but they also experience failures. Understanding failures in HRI is crucial for improving these systems. Prior study \citep{honig2018understanding} has identified two primary categories of robot failures: technical and interaction failures. Technical failures typically stem from hardware malfunctions or issues in the robot's software system, like communication issues. Interaction failures arise from uncertainties in interacting with humans or the environment, such as communication breakdowns and violations of social norms.
% \elmira{@Yooki add one/two studies related to failures in HRI, and the last sentence could be about the use of explanations for recovery }.
A study \citep{relatedwork_failure_3374782} investigated user perceptions of conversational failures in robots, demonstrating that humanoid robots enhance users' responses to such failures. Moreover, other studies show that explanations enhance recovery from failures; for instance, \citep{relatedwork_failure_3444657} demonstrated that explanations incorporating context and prior actions are most useful for non-expert users in diagnosing failures and identifying solutions.

\subsection{Explanations in HRI}
Robots' decision-making processes are often perceived as a ``black box,'' making explanations crucial for humans to better understand robotic behaviour \citep{relatedwork_explanation_han2021need}. Explanations have been shown to significantly shape cognitive perceptions, and they can be categorized into three types: \textit{what-explanations}, \textit{why-explanations}, and \textit{how-explanations}, depending on the content being explained \citep{relatedwork_explanation_MILLER20191}. A well-designed explanation enhances transparency in the robot’s operation, improving user understanding, particularly for non-expert users \citep{relatedwork_explanation_hayes2017improving}. For instance, robots with explanations are often perceived as more lively and human-like \citep{relatedwork_explanation_9900558}. However, an inadequate or unclear explanation can negatively affect user interaction \citep{relatedwork_explanation_3565480}.

When a robot behaves unexpectedly, often perceived as errors or failures, clear \textit{why-explanations} are frequently required \citep{relatedwork_explanation_3634990}. Additionally, prior research demonstrates that explanations contribute to the construction and repair of users' mental models, including their knowledge and understanding of the robot’s functions. These mental models potentially influence users’ expectations during interactions \citep{relatedwork_explanation_MILLER20191, relatedwork_explanation_hilton1996mental}.

Despite existing research, there is a significant gap in understanding how user expectations are shaped by priming and robot explanations within HRI contexts. Further investigation is needed to assess the effect of priming on user expectations and perceptions and to explore how the explanation influences these expectations throughout the interaction. 
% \yujing{not sure if we could state like this, since the priming and explanation will be introduced later, no idea where should I put this....}
% \elmira{for now I moved it here}

==> sections/03_Scenario_Design_and_Development.tex <==
\nopagebreak
\section{Scenario Design and Development}


\yujing{have moved Robot Capabilities and Failure to related work part}

\elmira{Add the details for the priming videos to the next section and the details about the main video to the main evaluation section}
% \subsection{Robot Capabilities}
% %\yujing{maybe we could add the pictures of these two robots here, or the setup scenario of the video containing these 2 robots}
% %\beatriz{on it!}
% %\yujing{since u already added the setup scenario with the 2 robots, maybe we could delete the Official website pictures to save some pages?...}
% \subsubsection{Pepper}
% % Pepper is a humanoid robot by SoftBank(REF) designed to interact with people in contexts such as customer service, retail, and educational environments. As a versatile platform, it is also used in research and education to explore human-robot interaction and social robotics. The pepper robot is a mobile robot with two HD 5-megapixel cameras (mouth and forehead), 3D sensor (behind eyes), four microphones, and three touch sensors REF. Torso with a gyroscope, and with two touch sensors REF. Leg/mobile base with two sonars, six lasers, three bumper sensors, and a gyroscope REF. It is able to move its body to complete various tasks, but its facial expression is always the same. Pepper runs on an open and programmable platform, utilizing a NAOqi operating system. It supports Python, C++, Java, JavaScript, and ROS interface. It connects to Android Studio via its software development kit (SDK) and Pepper SDK  REF. 
% Pepper \citep{softbankpepper} is a humanoid robot developed by SoftBank for interaction scenarios in customer service, retail, and educational settings. It is equipped with cameras, a 3D sensor, and microphones, allowing it to perceive its surroundings and respond verbally or bodily. Besides, with the mobile base and flexible body structure, it can move around, adopt various postures, and hold objects. However, Pepper’s face remains static, with no facial expressions or mouth movements during speech.


% \subsubsection{Furhat}
% % Furhat is a conversational robot by Furhat robotics (REF) with a back projected face. This robot is composed of a bust with onboard camera sensor and microphones, an LED ring  and is able to convey facial expressions and natural movements such as nodding, head-shaking and raising eyebrows (REF).The Furhat Platform has a library of faces of different gender, ages, skin colours, and human likeness, as well as a large selection of voices with different speaking styles (REF). The Furhat SDK includes a virtual Furhat with a complete environment to simulate interactions and a set of tools for creating gestures, logging and wizard-of-Oz.(REF)

% Furhat \citep{furhatrobotics}, developed by Furhat Robotics, is a conversational robot with a 3D printed face that can be changed physically and featuring a back-projected face capable of displaying a wide range of facial expressions. It allows customization of its appearance, offering options for different genders, ages, skin tones, and voices with varied speaking styles. Furhat could show natural head movements and facial expressions such as nodding, shaking, and raising eyebrows. However, being a head-shaped robot, Furhat cannot move or display body postures.


% % \subsubsection{Pepper}
% % Pepper \citep{softbankpepper} is a humanoid robot developed by SoftBank for interaction scenarios in customer service, retail, and educational settings. It is equipped with cameras, a 3D sensor, and microphones, allowing it to perceive its surroundings and respond verbally or bodily. Besides, with the mobile base and flexible body structure, it can move around, adopt various postures, and hold objects. However, Pepper’s face remains static, with no facial expressions or mouth movements during speech.

% % \subsubsection{Furhat} Furhat \citep{furhatrobotics}, developed by Furhat Robotics, is a conversational robot with a human face, featuring a back-projected face capable of displaying a wide range of facial expressions. It allows customization of its appearance, offering options for different genders, ages, skin tones, and voices with varied speaking styles. Furhat could show natural head movements and facial expressions such as nodding, shaking, and raising eyebrows. However, being a head-shaped robot, Furhat cannot move or display body postures.
% % }

% \subsection{Robot Failures}
% We utilized the taxonomy of failures proposed by \citep{honig2018understanding} (Figure \ref{tax}) to guide the development of our scenarios. This taxonomy distinguishes between two primary categories of failures: technical failures and interaction failures. Technical failures arise from hardware malfunctions or issues within the robot's software system. Interaction failures, on the other hand, stem from uncertainties in interactions with the environment, other agents, or humans, and include issues such as social norm violations and various forms of human error. We selected three error types for the priming videos—\textit{communication failures}, \textit{hardware failures}, and \textit{social norm violations}—as these are directly attributable to the robot and are visually demonstrable in a video format.

% \begin{figure}[htp]
%     \c6entering
%     \includegraphics[width=0.48\textwidth]{figures/taxonomy.jpg}
%     \caption{A human-robot failure taxonomy. Adapted from \citep{honig2018understanding}.}
%     \label{tax}
% \end{figure}


\subsection{Scenario Design}
%In the scenario design, we intentionally created distinct contexts for the priming videos and the main task videos to emphasize a clear differentiation between the two. For the negative priming videos, as well as the main task videos with and without explanations, we depicted the same types of errors.
To ensure consistency and minimize the potential influence of video format on results, both the priming and main task videos were designed with similar visual and technical settings (Figure \ref{fig:video_setting}). Each video featured two human actors and one robot (either Pepper or Furhat). However, to clearly distinguish between priming and main task videos, different actors and scenario settings were used. Importantly, the scenarios presented in the priming and main task videos were independent and not consequential to one another. Both the priming and main task videos incorporated the same types of errors—communication failures, hardware malfunctions, and social norm violations—based on the human-robot failure taxonomy outlined earlier. Each video had a duration of approximately two minutes, and subtitles were added.

\subsubsection{Priming Videos} 
%The priming videos were designed to either highlight the robots' success or failure in task execution within a specific context, thereby influencing participants' expectations (Table \ref{tab:priming_video_design}). The videos were set in a restaurant scenario, featuring a robot waiter (Pepper version) or a robot tasked with rating service quality (Furhat version). In both cases, the goal was to illustrate three types of errors: communication failures, hardware malfunctions, and social norm violations. Given the differing capabilities of the two robots, these errors were depicted in distinct ways, yet as similarly as possible to maintain consistency across different participant groups.
%For Pepper, the negative priming video begins with the robot interrupting a conversation between two customers by passing through the middle of their discussion. After guiding them to their table, Pepper returns to take their orders but fails to understand them correctly. Finally, when delivering the food, Pepper malfunctions and shuts down, causing the food to fall to the floor.
%For Furhat, the video starts with the robot repeatedly asking the customers to move closer after failing to detect them. It then interrupts the customers' conversation while asking another question, and finally, the robot shuts down before completing the last question.
%The positive priming videos for both robots followed the same structure as the negative ones but without any errors, allowing participants to observe how the robots would behave when functioning properly. Each video lasted approximately two minutes, and subtitles were added for clarity.

The priming videos were designed to influence participants' expectations by showcasing the robots' performance in task execution, either focusing on success or failure (Table \ref{tab:priming_video_design}). The priming videos were set in a restaurant context: in the Pepper version, the robot served as a waiter, while in the Furhat version, the robot was tasked with evaluating service quality. In both versions, the three predefined error types were consistently portrayed, either as full successes or complete failures. Although the errors were depicted according to each robot’s unique capabilities, the scenarios were designed to be as comparable as possible to maintain uniformity across participant groups. The positive priming videos followed the same structure but without any errors, allowing participants to observe how the robots performed when functioning correctly.


%\yujing{maybe use this code for table:}

\begin{table}[ht]
    \centering
    \caption{The priming videos design}
    \label{tab:priming_video_design}
    \begin{tabularx}{0.495\textwidth}{|m{0.75cm} | m{0.85cm}|m{1.85cm} |m{1.6cm}|m{1.75cm} |}
        \toprule
        \textbf{Robot} & \textbf{Priming} & \textbf{Communication failures} & \textbf{Hardware malfunctions} & \textbf{Social norm violations} \\ 
        \hline\hline
        \multirow{2}{=}{\textbf{Furhat}} 
        & \textit{Positive} 
        & Speaks properly
        & Completes the task
        & Robot understands\\
        \cline{2-5}
        & \textit{Negative} 
        & Fails to understand verbal cue
        & Shuts down and cannot finish instructions
        & Robot asks you to come closer and closer\\ 
        \hline\hline
        \multirow{2}{=}{\textbf{Pepper}} 
        & \textit{Positive} 
        & Speaks properly
        & Completes task
        & Keeps a proper social distance\\
        \cline{2-5}
        & \textit{Negative} 
        & Fails to understand verbal cue
        & Shuts down in the middle of the task
        & Passes in the middle of two people talking\\ 
        \bottomrule
    \end{tabularx}
\end{table}





\subsubsection{Main Task Videos}
% \yujing{maybe with the form, we do not need to detailedly describe with each scenario, but I am not sure...}
% The main task videos were designed to depict the robots' failures in task execution, either with or without an accompanying explanation (Table \ref{tab:main_video_design}). The videos were set in a museum scenario, featuring a robot guide (Pepper version) or a robot responsible for rating service (Furhat version). In both cases, the goal was to illustrate the same three types of errors as in the priming stage. Due to the robots' differing capabilities, these errors were portrayed differently but kept as consistent as possible, as they would be shown to different participants.
% For Pepper, the video (Figure \ref{pepvid}) begins with the robot speaking while facing the wrong direction during its task of guiding visitors through the exhibition. In the version with explanations, Pepper justifies the error by stating, "Sorry, I couldn’t recognize where you are because there is a problem with my camera." It later fails to realize that a visitor is still speaking, explaining, "Sorry, I couldn’t recognize you were still talking because your voice is too low." Finally, the robot fails to deliver an audio guide, dropping it.
% For Furhat, the video begins with the robot failing to detect the presence of people, explaining, "Sorry, I couldn’t recognize where you are because you are too far away." It then fails to acknowledge that the visitors are still speaking, providing the explanation, "Sorry, I couldn’t recognize you were still talking because your voice is too low." In the final instance, Furhat struggles with delivering its last question and explains, "Sorry, I am having problems with my motor functions, which is affecting my speech."
% In the videos without explanations, the same errors are depicted but without any rationale provided for the failures. Each video lasted approximately two minutes, with subtitles added for clarity.

The main task videos were intended to investigate the effect of explanations accompanying robot failures (Table \ref{tab:main_video_design}). These videos were set in a museum context: Pepper acted as a museum guide, and Furhat took on the role of a robot rating service. Both versions featured the same three error types as in the priming videos, but different specific errors were introduced to differentiate the main task videos. In the videos where an explanation was provided, the robot expressed an apology and offered a brief one-sentence explanation of the reason behind the error, aiming to help participants better understand the failure. For detailed settings and error types, refer to Table \ref{tab:main_video_design}.

%\yujing{maybe you can also try this code}
\begin{table}[ht]
    \centering
    \caption{The main video design}
    \label{tab:main_video_design}
    \begin{tabularx}{0.487\textwidth}{| m{0.78cm} | m{2.8cm} | m{4cm} |}
        \toprule
        \textbf{Robot} & \textbf{Failure} & \textbf{Explanation} \\ 
        \hline\hline
        \multirow{3}{=}{\textbf{Furhat}} 
        & Looking at the other direction while speaking
        & "Sorry, I couldn't recognize where you are because you are too far away"\\
        \cline{2-3}
        & Speaking over a person
        & "Sorry, I couldn't recognize you were still talking because your voice is too low"\\
        \cline{2-3}
        & Talking to a person and the voice gets un-understandable
        & "Sorry, I am having problems with my motor functions, which is affecting my speech" \\
        \hline\hline
        \multirow{3}{=}{\textbf{Pepper}} 
        & Looking at the other direction while speaking
        & "Sorry, I couldn’t recognize where you are because there is a problem with my camera.”\\
        \cline{2-3}
        & Speaking over a person
        &  ”Sorry, I couldn’t recognize you were still talking because your voice is too low.”\\
        \cline{2-3}
        & Dropping an object while carrying it
        & "Sorry, the object was too heavy for me to carry"\\
        \bottomrule
    \end{tabularx}
\end{table}


% \begin{figure}[htp]
%     \centering
%     \includegraphics[width=0.45\textwidth]{figures/peppervid.png}
%     \caption{\textbf{Pepper main task video frame.}}
%     \label{pepvid}
% \end{figure}

% \begin{figure}[htp]
%     \centering
%     \includegraphics[width=0.45\textwidth]{figures/furhatvid.png}
%     \caption{\textbf{Furhat main task video frame.}}
%     \label{furvid}
% \end{figure}

==> sections/08_Conclusion.tex <==
\section{Conclusion}
